Static Communication Analysis for Hardware Design

Hardware acceleration of algorithms is an effective method for improving performance in high-demand computational tasks. However, developing hardware designs for such acceleration fundamentally differs from software development, as it requires a deep understanding of the highly parallel nature of the hardware architecture. In this paper, we present a framework for the static analysis of communication within datapath architectures designed for field-programmable gate arrays (FPGAs). Our framework aims to enhance hardware design and optimization by providing insights into communication patterns within the architecture, which are essential for ensuring efficient data handling.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{Farzaneh Derakhshan \& Jan Hoffmann (Eds.): 16th International\\ Workshop on
Programming Language Approaches to Concurrency\\
and Communication-cEntric Software 2025 (PLACES 2025)\\
EPTCS 420, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.420.4}{10.4204/EPTCS.420.4}}
\pdfoutput=1

